Declarative Demand-Driven Reverse Engineering

Binary reverse engineering is a challenging task because it often necessitates reasoning using both domain-specific knowledge (e.g., understanding entrypoint idioms common to an ABI) and logical inference (e.g., reconstructing interprocedural control flow). To help perform these tasks, reverse engineers often use toolkits (such as IDA Pro or Ghidra) that allow them to interactively explicate properties of binaries. We argue that deductive databases serve as a natural abstraction for interfacing between visualization-based binary analysis tools and high-performance logical inference engines that compute facts about binaries. In this paper, we present a vision for the future in which reverse engineers use a visualization-based tool to understand binaries while simultaneously querying a logical-inference engine to perform arbitrarily-complex deductive inference tasks. We call our vision declarative demand-driven reverse engineering (D^3RE for short), and sketch a formal semantics whose goal is to mediate interaction between a logical-inference engine (such Souffle) and a reverse engineering tool. We describe aprototype tool, d3re, which are using to explore the D^3RE vision. While still a prototype, we have used d3re to reimplement several common querying tasks on binaries. Our evaluation demonstrates that d3re enables both better performance and more succinct implementation of these common RE tasks.

==> Makefile <==

PACKAGE=paper

PDF = $(PACKAGE).pdf

all:  ${PDF}

%.pdf:  %.tex
	pdflatex $<
	- bibtex $*
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

clean:
	$(RM)  *.pdf *.aux *.log *.bbl *.blg *#* *~*

.PHONY: all docclean clean archive zip


==> related.tex <==
\section{Related Work}
\label{sec:related}

\subsection{Logic program in reverse engineering}

Few work is done in combining logic programming and reverse engineering. Unlike
\tool{} most existing work still mainly focused on some specific problems, but not
a general tool that can deal with a broad kind of reverse engineering problem.
OOAnalyzer\cite{schwartz:2018} is one of them, it is a tool designed to recover
C++ abstraction in a binary using logic programming language. It also provides a
Ghidra plugin currently, but it will only work for programs originally written
in C++. Most of the rules in OOAnalyzer are based on win32 thiscall calling
convention, so it is also not easy to be directly used it for binaries in linux
and other platforms.

XSB-Prolog is chosen as the logic engine of OOAnalyzer. In order to achieve good
performance and make sure forward reasoning always terminates, all rules in
OOAnalyzer are running in tabling mode\cite{swift:2010}. In \tool{}, we choose
datalog as our logic engine. Datalog is similar to prolog with tabling, the
semantic of datalog guaranteed termination of a program for free. In performance
perspective, nowadays datalog engines like souffle have much better performance
compared to prolog implementations like XSB-prolog, SWI-prolog.


% \subsection{Disassembler}

% The very first step of reverse engineering is disassembling . There are many
% good works in this area such as captone, uroboros and ramblr.
% Ddisasm\cite{floresmontoya:2020} is one of them. It introduces datalog into this
% area to make decompilation more precise. Firstly it uses capstone doing linear
% disassembling at any possible offset inside a binary to get a super set of
% possible assemble code, and then implement some static analysis like value
% analysis, register use-def analysis in datalog to eliminate conflicts and error
% in code. Although some of the rules used in Ddisasm are heuristic which means it
% is not 100\% precise, the result of Ddisasm is still better than other
% disassemblers. In order to do further reverse on assembly code using datalog,
% disassembly results must be encoded into facts. Since DDisasm is a datalog
% system, the output of it’s datalog rule can be directly used as input for the
% next stage. \tool{} use ddisasm as disassembler backend and store all intermediate
% facts generated by Ddisasm. When using \tool{}, users can have access to all rules
% declared in ddisasm.

% Gigahorse\cite{ngrech:2019} is another decompiler using datalog, but their work
% targets blockchain application decompilation. Instead of generating assembly
% code like a normal decompiler, it will generate EVM bytecode. Our work will
% still focus on x86 and x64 architecture binary.

\subsection{Program Analysis Using Datalog}

There is lots of good research in high performance datalog compilers. Due to
proper data structure and good index selection algorithm \cite{subotic:2018},
the speed of souffle is really fast. Compared to other datalog implementations,
souffle has a good debugger and abundant language features like arithmetic and
component. These features are very useful for design program analysis algorithms
using datalog. In souffle’s source code repository, it gives lots of examples of
how to do small size of program analysis, but it is also applicable for large
size program analysis .Most famous program analysis framework using datalog is
Doop \cite{smaragdakis:2014}. Doop is a pointer analysis framework that allows
users to do object sensitive analysis on large size java programs like tomcats.
And in the binary analysis area, OOAnalyzer also shows using logic program
language like datalog and prolog can make analysis both more readable and
faster.


